Local Rademacher Complexity-based Learning Guarantees for Multi-Task Learning

We show a Talagrand-type concentration inequality for Multi-Task Learning (MTL), using which we establish sharp excess risk bounds for MTL in terms of distribution- and data-dependent versions of the Local Rademacher Complexity (LRC). We also give a new bound on the LRC for norm regularized as well as strongly convex hypothesis classes, which applies not only to MTL but also to the standard i.i.d. setting. Combining both results, one can now easily derive fast-rate bounds on the excess risk for many prominent MTL methods, including---as we demonstrate---Schatten-norm, group-norm, and graph-regularized MTL. The derived bounds reflect a relationship akeen to a conservation law of asymptotic convergence rates. This very relationship allows for trading off slower rates w.r.t. the number of tasks for faster rates with respect to the number of available samples per task, when compared to the rates obtained via a traditional, global Rademacher analysis.

==> Acknowledgments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Acknowledgements should only appear in the accepted version. 
\section*{Acknowledgments} 



==> Applications.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Applications}
\label{sec:Applications}
As an application of \thrmref{MainTheorem}, we present the (distribution-dependent) excess risk bound for a pair of hypothesis spaces intended to be used in the context of \ac {MTL} binary classification. Note that, with the help of \thrmref{MainTheorem2}, the data-dependent version of the excess risk bounds can be obtained in the same way. A theoretically well-studied \ac {MTL} framework is the regularized linear \ac {MTL} model, in which each function $f_t$ is featured as a linear function with weight $\boldsymbol{w}_t \in \mathcal{H}$, such that $\forall X \in \mathcal{X} \subset \mathcal{H}, f_t(X) = \left\langle  \boldsymbol{w}_t, X \right\rangle $, where $\mathcal{H}$ is a real Hilbert space equipped with inner product $\left\langle  .,. \right\rangle $. Different regularizers can be employed to model information sharing between different tasks. In this study, we consider the framework in which the tasks are implicitly related by a regularizer on $\boldsymbol{W} = (\boldsymbol{w}_1, \ldots, \boldsymbol{w}_T) \in \mathcal{H} \times \ldots \times \mathcal{H}$. Formally, given $\{X_t^{i},Y_t^{i}\}_{(i,t)=(1,1)}^{(n,T)} \in {\mathcal{X}, \mathcal{Y}}$, where $\mathcal{X}$ and $\mathcal{Y}$ are the input and output space for each task, the framework can be written as
\begin{align}
\label{MTLGeneralModel}
\min_{\boldsymbol{W}} R(\boldsymbol{W}) + \lambda \sum_{i,t} \ell \left( f_t(X_t^{i}), Y_t^{i}\right) 
\end{align} 
\noindent
where $R(.)$ and $\ell(.,.)$ are the regularizer and loss function, respectively. Now, let us present the following Proposition\footnote{Note that \propref{Propos:Proposition1} here utilizes the first part of Proposition 12 in \cite{kloft2011lp} and does not require the strong duality assumption, which is necessary for the second part of Proposition 12 in \cite{kloft2011lp}} which help us to identify the hypothesis space of any \ac {MTL} model in the form of \eqref{MTLGeneralModel} which we will study in this section. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Proposition %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[Proposition 12 in \cite{kloft2011lp}, part (a)]
\label{Propos:Proposition1}
Let $\mathcal{C} \subseteq \mathcal{X}$ and let $f, g: \mathcal{C} \mapsto \mathbb{R}$ be two functions. For any $\nu > 0$, there must exist a constant $\eta > 0$, such that the optimal solution of \eref{Klof-first part1} is also optimal for \eref{Klof-first part2}  
\begin{align}
\label{Klof-first part1}
\min_{x \in \mathcal{C}} f(x)+\nu g(x)\\
\label{Klof-first part2}
\min_{x \in \mathcal{C}, g(x) \leq \eta} f(x)
\end{align}
\end{prop}
\noindent
The proof of this Proposition can be found in \cite{kloft2011lp}. 

Using \propref{Propos:Proposition1}, one can show that Problem \eqref{MTLGeneralModel} is equivalent to the following problem:

\begin{align}
	& \min_{\boldsymbol{W}\in\varOmega\left( \boldsymbol{W}\right)} \ C \sum_{t=1}^{T}\sum_{i=1}^{n} \ell \left( f_{t} (X_{t}^{i}) ,Y_t^i\right)
	\nonumber\\
    \varOmega \left( \boldsymbol{W}\right)  :=  &
	\lbrace \boldsymbol{W} =  \left[ \boldsymbol{w}_1,\cdots,\boldsymbol{w}_T\right] : \;  R\left(  \boldsymbol{W} \right) \leq R \rbrace 
	\nonumber
\end{align}
\noindent
Therefore, its relevant hypothesis space can be defined as 
\begin{align}
\label{GeneralHSForFixedMApping}
\mathcal{F} := \left\lbrace  X \mapsto [\left\langle \boldsymbol{w}_1, X_1 \right\rangle , \ldots, \left\langle \boldsymbol{w}_T, X_T \right\rangle ]^{T} : R\left(  \boldsymbol{W} \right) \leq R \right\rbrace. 
\end{align}

In this section we consider a number of interesting \ac {MTL} models with a regularizer of matrix $\boldsymbol{W} = [\boldsymbol{w}_{1}, \ldots, \boldsymbol{w}_{T}]$. More specially, we consider the following formulation with a preselected fixed kernel $k: \mathcal{X} \times \mathcal{X} \mapsto \mathbb{R}$ and corresponding feature mapping $\phi: \mathcal{X} \mapsto \mathcal{H}$
\begin{align}
\label{GeneralFixedMappingModel}
\min_{\boldsymbol{W}}  R \left(  \boldsymbol{W} \right)   +  C \sum_{t=1}^{T}  \sum_{i=1}^{n} \ell( \left\langle \boldsymbol{w}_t , \phi(X_t^{i})\right\rangle_{\mathcal{H}} , Y_t^{i}), 
\end{align}
\noindent
where $ R \left(  \boldsymbol{W} \right)$ is a matrix norm of $\boldsymbol{W}$. 

%Using \propref{Propos:Proposition1}, one can show that Problem \eqref {GeneralFixedMappingModel} is equivalent to the following problem:
%
%\begin{align}
%	& \min_{\boldsymbol{W}\in\varOmega\left( \boldsymbol{W}\right)} \ C \sum_{t=1}^{T}\sum_{i=1}^{n} l\left( \boldsymbol{w}_t,\phi\left( X_t^i \right),Y_t^i\right)
%	\nonumber\\
%    \varOmega \left( \boldsymbol{W}\right)  :=  &
%	\lbrace \boldsymbol{W} =  \left[ \boldsymbol{w}_1,\cdots,\boldsymbol{w}_T\right] : \;  R\left(  \boldsymbol{W} \right) \leq R \rbrace 
%	\nonumber
%\end{align}
%\noindent
%Therefore, its relevant hypothesis space can be defined as 
%\begin{align}
%\label{GeneralHSForFixedMApping}
%\mathcal{F} := \left\lbrace  X \mapsto [\left\langle \boldsymbol{w}_1, \phi (X_1)\right\rangle , \ldots, \left\langle \boldsymbol{w}_T, \phi (X_T)\right\rangle ]^{T} : R\left(  \boldsymbol{W} \right) \leq R \right\rbrace. 
%\end{align}

In the sequence, we include various common \ac {MTL} formulations based on the group norm, Schatten norm and graph regularizers of $\boldsymbol{W}$ \cite{maurer2006Graph,evgeniou2007,argyriou2007,argyriou2008,li2013,argyriou2014Graph}

%On the other hand, another angle of considering information sharing amongst tasks is by preprocessing the data from all tasks by a common processor, and subsequently, a linear model is learned based on the processed data. One scenario of this learning framework is subspace learning, where data of each task are projected to a common subspace by an operator $A$, and then the $\boldsymbol{w}_t$s are learned in that subspace. Another particularly straightforward and useful adaptation of this framework is kernel-based \ac {MTL}. In this situation, the role of the operator $A$ is assumed by the nonlinear feature mapping $\phi$ associated with the kernel function in use. In this case, all data are preprocessed by a common kernel function, which is preselected or learned during the training phase, while the $\boldsymbol{w}_t$s are then learned in the \ac{RKHS}.

%Given a set $A$ of bounded self-adjoint linear operators on $\mathcal{X}$ and $T$ linear functions with weights $\boldsymbol{w}_t$s, the \ac {HS} is given as $\mathcal{F} = \{X \mapsto [\left\langle  \boldsymbol{w}_1, AX_1 \right\rangle , \ldots \left\langle \boldsymbol{w}_T, AX_T\right\rangle ]^{'} : \| \boldsymbol{w}_t \|^{2}  \leq R,  A \in \mathcal{A} \} $. Clearly, in this \ac {HS}, data are preprocessed by the operator $A$ to a common space, as a strategy of information sharing amongst tasks. By either cleverly choosing $A$ beforehand or by learning $A \in \mathcal{A}$, it is expected that a tighter generalization bound can be attained compared with learning each task independently. It is straightforward to see that preselecting $A$ beforehand is a special case of learning $A \in \mathcal{A}$, \ie, preselecting $A$ is equivalent to $\mathcal{A} = \{A \}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Fixed Feature Mapping %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{\ac {MTL} Approaches with a Fixed Feature Mapping}
%\label{ssec:FixedfeatureMapping}
%In this section we consider a number of interesting \ac {MTL} models with a matrix-based regularization function of matrix $\boldsymbol{W} = [\boldsymbol{w}_{1}, \ldots, \boldsymbol{w}_{T}]$. This includes various common \ac {MTL} formulations based on group norm, Schatten norm and graph regularizers \cite{argyriou2007,argyriou2008,li2013,maurer2006Graph}. Consider the following \ac {MTL} formulation with a preselected fixed kernel $k: \mathcal{X} \times \mathcal{X} \mapsto \mathbb{R}$ and corresponding feature mapping $\phi: \mathcal{X} \mapsto \mathcal{H}_{\phi}$
%\begin{align}
%\label{prob:GeneralFixedMappingModel}
%\min_{\boldsymbol{W}}  R\left(  \boldsymbol{W} \right)   +  C \sum_{t=1}^{T}  \sum_{i=1}^{n} l(\boldsymbol{w}_t , \phi(X_t^{i}) , Y_t^{i}), 
%\end{align}
%\noindent
%where $ R\left(  \boldsymbol{W} \right)$ is a matrix norm of $\boldsymbol{W}$.
%
%Using \propref{Propos:Proposition1}, one can show that Problem \eqref {prob:GeneralFixedMappingModel} is equivalent to the following problem:
%
%\begin{align}
%	& \min_{\boldsymbol{W}\in\varOmega\left( \boldsymbol{W}\right)} \ C \sum_{t=1}^{T}\sum_{i=1}^{n} l\left( \boldsymbol{w}_t,\phi\left( X_t^i \right),Y_t^i\right)
%	\nonumber\\
%    \varOmega \left( \boldsymbol{W}\right)  :=  &
%	\lbrace \boldsymbol{W} =  \left[ \boldsymbol{w}_1,\cdots,\boldsymbol{w}_T\right] : \;  R\left(  \boldsymbol{W} \right) \leq R \rbrace 
%	\nonumber
%\end{align}
%\noindent
%Therefore, its relevant hypothesis space can be defined as 
%\begin{align}
%\label{GeneralHSForFixedMApping}
%\mathcal{F} := \left\lbrace  X \mapsto [\left\langle \boldsymbol{w}_1, \phi (X_1)\right\rangle , \ldots, \left\langle \boldsymbol{w}_T, \phi (X_T)\right\rangle ]^{T} : R\left(  \boldsymbol{W} \right) \leq R \right\rbrace. 
%\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Group Norm Regularizer MTL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Group Norm Regularized \ac {MTL}}
\label{ssec:GroupNormRegularizer}
As an example of the case where the inter-task relationships are captured by imposing a group norm regularizer on $\boldsymbol{W}$ \cite{evgeniou2007,argyriou2008,lounici2009,romera2012}, we consider the $L_{2,q}$ which is defined here as 
\begin{align}
\label{GroupFixedMappingModel}
R(\boldsymbol{W}) =   \left\| \boldsymbol{W} \right\| _{2,q} =  \left\|  ( \left\|  \boldsymbol{w}_{1} \right\| _{2}, \ldots, \left\|  \boldsymbol{w}_{T} \right\| _{2} )\right\| _{q} = (  \sum_{t=1}^{T} \left\|  \boldsymbol{w}_t \right\| _{2} ^{q}  )^{1/q}.
\end{align}
\noindent
Then, using \propref{Propos:Proposition1}, one can show that the relevant hypothesis space for a \ac {MTL} problem with regularizer \eqref{GroupFixedMappingModel} is
\begin{align}
\label{GroupHSForFixedMApping}
\mathcal{F}_{q} := \left\lbrace  X \mapsto [\left\langle \boldsymbol{w}_1, \phi (X_1)\right\rangle , \ldots, \left\langle \boldsymbol{w}_T, \phi (X_T)\right\rangle ]^{T} : \left\| \boldsymbol{W} \right\| _{2,q} \leq R_{max} \right\rbrace 
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Schatten Norm Regularizer MTL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Schatten Norm Regularized \ac {MTL}}
\label{ssec:SchattenNormRegularizer}
Another interesting \ac {MTL} formulation which has been studied in \cite{argyriou2007} shows that, the shared structure between tasks can also be modeled using a function $F$ which forces a relatedness structure though a positive operator $\boldsymbol{D}$ which itself is a function of the task's covariance matrix $\boldsymbol{W}\boldsymbol{W}^{T}$. For this purpose, they propose the regularization function $tr (\boldsymbol{W}^{T} F(\boldsymbol{D}) \boldsymbol{W})$ in which the function $F$ is a prescribed negative power spectral function of the eigenvalues of its argument (denoted by $f$). They further show that the resulting regularization problem is equivalent to regularization with a Schatten $L_q$ prenorm of $\boldsymbol{W}$, when the coupling function $f$ takes the form $f(x) = x^{1-\frac{2}{q}}$ with $q \in (0,2]$. In a similar way, the hypothesis space of this problem can be obtained as 
\begin{align}
\label{HSForFixedMAppingSchatten}
\mathcal{F}_{S_q} := \left\lbrace  X \mapsto [\left\langle \boldsymbol{w}_1, \phi (X_1)\right\rangle , \ldots, \left\langle \boldsymbol{w}_T, \phi (X_T)\right\rangle ]^{T} :  \| \boldsymbol{W} \|_{S_q}  \leq R'_{max}, q \in (0,2] \right\rbrace. 
\end{align}
\noindent
where for $\left|  \boldsymbol{W} \right| = \sqrt{ \boldsymbol{W}^{T} \boldsymbol{W}}$,
\begin{align}
R(\boldsymbol{W}) =  \| \boldsymbol{W}\|_{S_q} := \left[ \text {tr} \left( \left|  \boldsymbol{W} \right| ^{q} \right) \right] ^{\frac{1}{q}}. 
 %:= \left\lbrace \sum_{i=1}^{\infty} \left( \lambda_{i} (\boldsymbol{W})\right)^{q}\right\rbrace^{\frac{1}{q}}  
 \nonumber
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Graph Regularizer MTL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Graph Regularized \ac {MTL}}
\label{:GraphRegularizer}
 The idea of graph regularization in \ac {MTL}  is to force the classifiers of related tasks to be close to each other by penalizing the squared distance $\| \boldsymbol{w}_{t} - \boldsymbol{w}_{s} \|^{2}$ proportional to $\omega_{ts}$. We consider the \ac {MTL} graph regularizer given in \cite{maurer2006Graph} as
\begin{align}
\label{GraphReg}
R (\boldsymbol{W}) = \frac{1}{2T} \sum_{t=1}^{T} \sum_{s=1}^{T} \omega_{ts} \| \boldsymbol{w}_{t} - \boldsymbol{w}_{s} \|^{2} + \frac{\eta}{T} \sum_{t=1}^{T} \| \boldsymbol{w}_{t} \|^{2} = \frac{1}{T} \sum_{t=1}^{T} \sum_{s=1}^{T} \left( \boldsymbol{L}+ \eta \boldsymbol{I}\right)_{ts} \left\langle \boldsymbol{w}_{t} , \boldsymbol{w}_{s}\right\rangle, 
\end{align}
\noindent
where $\boldsymbol{L}$ is the Laplacian of the graph with $T$ vertices and edge-weights $\omega$, $\boldsymbol{I}$ is the identity in $\mathbb{R}^{T}$, and $\eta > 0$ is the regularization parameter. It can be easily shown that $\frac{1}{T} \sum_{t=1}^{T} \sum_{s=1}^{T} \left( \boldsymbol{L}+ \eta \boldsymbol{I}\right)_{ts} \left\langle \boldsymbol{w}_{t} , \boldsymbol{w}_{s}\right\rangle  = (1/T) \text {tr} \left( \boldsymbol{W}^{T} (\boldsymbol{L}+ \eta \boldsymbol{I}) \boldsymbol{W} \right) = (1/T) \|  (\boldsymbol{L}+ \eta \boldsymbol{I})^{1/2} \boldsymbol{W} \|_{F}^{2}$. Therefore, using \propref{Propos:Proposition1}, the relevant hypothesis space for \ac {MTL} Problem \eqref{GeneralFixedMappingModel} with $R(\boldsymbol{W})$ defined as \eqref{GraphReg} and $\boldsymbol{D}= \boldsymbol{L} + \eta \boldsymbol{I}$ is given as
\begin{align}
\label{GraphRegHS}
\mathcal{F}_{G} := \left\lbrace  X \mapsto [\left\langle \boldsymbol{w}_1, \phi (X_1)\right\rangle , \ldots, \left\langle \boldsymbol{w}_T, \phi (X_T)\right\rangle ]^{T} :  \| \boldsymbol{D}^{1/2} \boldsymbol{W}\|_{F}  \leq R''_{max}\right\rbrace. 
\end{align}

In general, one can come up with the following \ac {MTL} formulation which can cover all the cases discussed above:
\begin{align}
\label{GeneralNormFormulation}
\min_{\boldsymbol{W}} R(\boldsymbol{W}) + \lambda \sum_{i,t} \ell \left( f_t(X_t^{i}), Y_t^{i}\right), 
\end{align}
\noindent
with $R(\boldsymbol{W})= \left\|\boldsymbol{D}^{1/2} \boldsymbol{W} \right\| $ and positive operator $\boldsymbol{D}$.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Different cases for positive operator D %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Note that if we set $\boldsymbol{D} = I$, by choosing the appropriate norms, we can retrieve the hypothesis spaces $\mathcal{F}_{q}$, $\mathcal{F}_{S_q}$. Also, if we set $\boldsymbol{D} = \boldsymbol{L} + \eta \boldsymbol{I}$, where $\boldsymbol{L}$ is the Laplacian on a graph with $T$ vertices, and $\eta > 0$ a small regularization constant, then the hypothesis space corresponding to the graph regularization scheme \eqref{GraphReg} can be obtained. 



==> Conclusions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}
\label{sec:Conclusions}



==> Experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Applications}
\label{sec:Applications}


==> TitleAuthors.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\MYTITLE}{Multi-Task Learning with Group-Specific\texorpdfstring{\\}{} Feature Space Sharing}

% The \ecmltitle you define below is probably too long as a header.
% Therefore, a short form for the running title is supplied here:
%\title{Multi-Task Learning with Unrestricted Task Affinity}
\title{\MYTITLE}

\author{Niloofar Yousefi\inst{1} \and Michael Georgiopoulos\inst{1} \and \\ Georgios C. Anagnostopoulos\inst{2}}

\institute{University of Central Florida, Department of Electrical Engineering \& Computer Science, 4000 Central Florida Blvd, Orlando, Florida, 32816, USA \\
\email{niloofar.yousefi@ucf.edu, michaelg@ucf.edu}
\and Florida Institute of Technology, Department of Electrical and Computer Engineering,\\ 150 W. University Blvd, Melbourne, FL 32901, USA \\
\email{georgio@fit.edu}}


